Do Code Review Measures Explain the Incidence of Post-Release Defects?

Aim: In contrast to studies of defects found during code review, we aim to clarify whether code reviews measures can explain the prevalence of post-release defects. Method: We replicate a study by McIntoshet. al that uses additive regression to model the relationship between defects and code reviews. To increase external validity, we apply the same methodology on a new software project. We discuss our findings with the first author of the original study, McIntosh. We then investigate how to reduce the impact of correlated predictors in the variable selection process and how to increase understanding of the inter-relationships among the predictors by employing Bayesian Network (BN) models. Context: As in the original study, we use the same measures authors obtained for Qt project in the original study. We mine data from version control and issue tracker of Google Chrome and operationalize measures that are close analogs to the large collection of code, process, and code review measures used in the replicated the study. Results: Both the data from the original study and the Chrome data showed high instability of the influence of code review measures on defects with the results being highly sensitive to variable selection procedure. Models without code review predictors had as good or better fit than those with review predictors. Replication, however, confirms with the bulk of prior work showing that prior defects, module size, and authorship have the strongest relationship to post-release defects. The application of BN models helped explain the observed instability by demonstrating that the review-related predictors do not affect post-release defects directly and showed indirect effects. For example, changes that have no review discussion tend to be associated with files that have had many prior defects which in turn increase the number of post-release defects.

==> other_text.tex <==
\subsection{Role of Expertise Measures in the Bayesian Network model.}
We found that the two expertise related variables, \emph{changes no expertise} (representing 
changes by authors lacking subject matter expertise) and 
\emph{typical reviewer expertise} (representing typical reviewer expertise) are not part 
of the Markov blanket of the \emph{defects} variable in our BN model. 
Thus, as expected, we found that adding these two variables did not 
change the results in any way. 



71.4
The number of distinct authors that have changed a directory, allauthors, the 
In only two of seven releases do review measures have a direct impact on defects in the Markov Blanket.  


In Qt combined, we have only two releases, so it is ....

HOwever, for Chrome when more releasees,

Across all releases we see no review measures. 
By examining the conditional probability tables (CPT) of \emph{defects}
and the variables in its Markov Blanket we can understand the extent of effect these variables have on 
post-release defects. We show the CPTs for the BN models for all individual the Qt
and Chrome releases, and the combined Qt and Chrome releases in Table \ref{t:cpt}.


The BN model with the combined data for all the releases showed a good accuracy (0.83) and fair Kappa value (0.45), and was able to explain 32.7\% of the variance in post-release defects, which leads us to believe that it is a good general model for explaining the number of post-release defects for both Chrome and Qt. When tested against the data for individual releases for the two projects, the variance explained, accuracy, and Kappa values for this model varied between 20.2\% and 35.7\%, 0.78 and 0.84, and 0.41 and 0.5 respectively. 

We combined the release data for each project, two releases for Qt and four for Chrome, and combine the data across projects into a single model. The reason for combining the datasets was twofold: firstly, we observed that the BN models for individual releases of both software were similar, which led us to believe that the underlying distribution for the observed variables was similar as well, so combining the releases did not violate any underlying assumptions, and secondly, combining the datasets make our final model more robust and the result more generalizable, because of having more training examples and not being prone to overfit to the specific characteristics of one particular release. The performance of the BN models, along with the variables that affect the number of post-release defects, is also shown in Table~\ref{t:MB_release}. The Kappa values for these models, similar to what we observed for the BN models for individual releases, showed a moderate amount of agreement, and the accuracy and variance explained by the models were also similar. 

% Although review related measures like \emph{allreviews}, \emph{allreviewers} 
% appeared in the Markov Blanket of the ``defects'' node for Chrome release 39 and 40
% respectively, they appeared only in those instances, and their effect was not seen 
% in the aggregated datasets, indicating their effects are comparatively small and
% did not affect the number of post-release defects across the releases. 
 
 can be for predictive or explanatory powerModels can be evaluated based on their predictive and explanatory
power, which are radically
different objectives~\cite{shmueli2010explain}.  Our main goal in this paper 
is to 

Model evaluation differs depending on the research goal~\cite{shmueli2010explain}. In this work, we are interested in explanatory models rather than predictive models. Our goal is to develop a model that explains how the software engineering measures explain post-release defects rather an predicting future defects. As a result, the magnitude
of \textit{variance explained}, as measured by the proportion of the log-likelihood score 
 relative to the baseline model of an empty graph that assumes all variables to be 
independent) by the model is an important performance measure for our models.  

% \begin{table}[t!]
% \centering
% \caption{CPT of \emph{defects} with the variables in its Markov blanket for BN model of all Chrome and Qt releases combined. For example with no minor authors there is a 23.3\% chance of there being postrelease defect(s), with 1 or more minor authors the probability rises to 41.7\%}
% \label{t:cpt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lll||lll||lll}
% size & \multicolumn{2}{l||}{defects} & minorauthors & \multicolumn{2}{l||}{defects} & priordefects & \multicolumn{2}{l}{defects} \\ \hline
%  & 0 & 1 &  & 0 & 1 &  & 0 & 1 \\
% {[}  0,   114) & 0.839 & 0.161 & 0 & 0.767 & 0.233 & {[}0, 2) & 0.926 & 0.074 \\
% {[}114,   571) & 0.735 & 0.265 & {[}1,108{]} & 0.583 & 0.417 & {[}2, 8) & 0.776 & 0.224 \\
% {[}571,106595{]} & 0.655 & 0.345 &  &  &  & {[}8,1702{]} & 0.439 & 0.561    \\\hline
% \end{tabular}
% }
% \vspace{-10pt} 
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
